Grain Growth During Protostellar Disk Formation

Recent observations indicate that mm/cm-sized grains may exist in the embedded protostellar disks. How such large grains grow from the micron size (or less) in the earliest phase of star formation remains relatively unexplored. In this study we take a first step to model the grain growth in the protostellar environment, using two-dimensional (2D axisymmetric) radiation hydrodynamic and grain growth simulations. We show that the grain growth calculations can be greatly simplified by the "terminal velocity approximation", where the dust drift velocity relative to the gas is proportional to its stopping time, which is proportional to the grain size. We find that the grain-grain collision from size-dependent terminal velocity alone is too slow to convert a significant fraction of the initially micron-sized grains into mm/cm sizes during the deeply embedded Class 0 phase. Substantial grain growth is achieved when the grain-grain collision speed is enhanced by a factor of 4. The dust growth above and below the disk midplane enables the grains to settle faster towards the midplane, which increases the local dust-to-gas ratio, which, in turn, speeds up further growth there. How this needed enhancement can be achieved is unclear, although turbulence is a strong possibility that deserves further exploration.

==> old-g-to-d.tex <==
\subsubsection{Dust-to-gas ratio and dust size layering}
\label{sec:g2d_dust_size_layer}

For the eventual formation of planets, one important quality to characterize is the dust-to-gas ratio since a high ratio is required to form planetesimals through streaming instability. We seek to understand the dust-to-gas ratio in our simulation. {\color{red}We would like to point out that because the gas and dust dynamics are calculated by two distinct algorithm, quantitative results can be affected by slightly numerical issues and should be treated as estimates to true values. Most of the results we present here are qualitative, and holds independent of numerical effects.}

In figure \ref{fig:gas_to_dust_ratio}, we show the normalized dust-to-gas ratio using the mass of all grains combined. We see a dust concentration on the disk midplane, where the dust-to-gas ratio is increased by a factor of 1.5 to 4. Such region exists in both panels of figure \ref{fig:gas_to_dust_ratio}, meaning this dust-to-gas ratio exists throughout our simulation as long as the disk is present. This increase will be important when we discuss why the grains grow on the disk midplane in section \ref{sec:sol_to_smoluchowski}. The dust-to-gas ratio being about 0.01 (the initial value) everywhere else in the disk suggests that most of the dust masses in other parts of the disk are well-coupled to the gas, so differential drift between gas and dust doesn't change the dust-to-gas ratio much. This well-coupling means that most of the grains have small stopping times - the grains are still small and not much growth has happened yet. Since we are interested in exploring grain growth in this work, we will focus on the disk midplane for the subsequent discussion.

In figure \ref{fig:midplane_grains_theta} we show the dust concentration as a function of radius on the midplane for each bin $>1\mu$m in our simulation, and annotate the location where the concentration is at an extremum (the dots on each line). We see that at locations >30AU, the dust concentration maximum radius increases monotonously as the grain size decreases. This finding can be a pure consequence of differential drift, as the maximum concentration can be expected to be closer to the center due to faster radial drift. A similar behavior is observed between 10 and 30AU, where the explanation can be similar to the outer one, but the existence of an inner concentration can also be a numerical effect of having a boundary at 10 AU.

In figure \ref{fig:midplane_grains_theta} we also plot the total grain density divided by 10 and gas density divided by 1000. Initially when dust-to-gas ratio is 0.01, these two line coincide perfectly. When the disk grows to 250AU, the maximum dust-to-gas radio increases to {\color{red} 0.034}. Later the maximum dust-to-gas ratio on the midplane increases to around 0.05 near the inner boundary. Although this dust to gas ratio of 0.05 is probably not enough to trigger streaming instability \citep{YoudinGoodman2005}, but if there are some radial support against grains losting to the central protostar due to radial drift, increasing dust-to-gas ratio to and above 0.1 (approximate streaming instability threshold) \citep{YoudinGoodman2005} isn't unreasonable. We defer this effect to future studies.
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{figures/74_40norm_dust_to_gas_ratio_2panels.png}
    \caption{dust-to-gas ratio on the meridian plane at two times, as specified in the title. Dust-to-gas of 0.01 is the ISM value; a value larger than 0.01 means there is a grain concentration and a smaller value implies a grain deficit. There is a concentration on the disk midplane as observed in the 88750 year frame, where the highest concentration has been increased to $\sim 3.5$. This higher concentration region has been observed to exist at least since 61500 years, at which time the high concentration region is around 25AU. This time scale of over 20000 years is important for our discussion in section \ref{sec:sol_to_smoluchowski}.}
    \label{fig:gas_to_dust_ratio}
\end{figure*}
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{figures/74_40_midplane_grains_theta_ind103.png}
    \caption{Grain density of grains of different sizes as a function of radius on the midplane. Lines of each color is the grain density of grains with size shown in the color bar. The dots with the same color at each lines shows a local density maxima of grains of that size. To compute these local maximas, the lines are smooth by replacing the values at each location with the three-point-average around that point to reduce the giggling in lines due to numerical effects (smoothed lines are not shown). The local maximas are then found numerically. Some of the dots located below $10^{-16}$g/cc and within $50$AU are present for numerical reasons. The upmost dots with varying color starting around $\sim30$AU shows the location of local maxima is monotone as a function of grain size. The black line is the sum of grain density over all size bins divided by 10 (to fit in the plot) and the gray line is the gas density divided by 1000. The initial gas-to-dust ratio of 100 will have the black and gray overlap on top of each other exactly, and the gas-to-dust ratio decreases below 100 within $\sim90$AU on the midplane.}
    \label{fig:midplane_grains_theta}
\end{figure*}

==> old_biblio.tex <==
@ARTICLE{Shu1977,
       author = {{Shu}, F.~H.},
        title = "{Self-similar collapse of isothermal spheres and star formation.}",
      journal = {\apj},
     keywords = {Density Distribution, Gravitational Collapse, Isothermal Flow, Protostars, Star Formation, Stellar Structure, Critical Point, Runge-Kutta Method, Similarity Theorem, Steady State, Stellar Envelopes, Astrophysics},
         year = 1977,
        month = jun,
       volume = {214},
        pages = {488-497},
          doi = {10.1086/155274},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1977ApJ...214..488S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hosokawa&Omukai2009,
       author = {{Hosokawa}, Takashi and {Omukai}, Kazuyuki},
        title = "{Evolution of Massive Protostars with High Accretion Rates}",
      journal = {\apj},
     keywords = {accretion, accretion disks, stars: early-type, stars: evolution, stars: formation, stars: pre-main sequence, Astrophysics},
         year = 2009,
        month = jan,
       volume = {691},
       number = {1},
        pages = {823-846},
          doi = {10.1088/0004-637X/691/1/823},
archivePrefix = {arXiv},
       eprint = {0806.4122},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009ApJ...691..823H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Laor&Draine1993,
       author = {{Laor}, Ari and {Draine}, Bruce T.},
        title = "{Spectroscopic Constraints on the Properties of Dust in Active Galactic Nuclei}",
      journal = {\apj},
     keywords = {Active Galactic Nuclei, Astronomical Models, Astronomical Spectroscopy, Computational Astrophysics, Cosmic Dust, Emission Spectra, Grain Size, Graphite, Interstellar Extinction, Optical Properties, Optical Thickness, Silicon Carbides, Astrophysics, ISM: DUST, EXTINCTION, GALAXIES: ACTIVE, GALAXIES: NUCLEI, INFRARED: INTERSTELLAR: LINES, RADIATIVE TRANSFER},
         year = 1993,
        month = jan,
       volume = {402},
        pages = {441},
          doi = {10.1086/172149},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1993ApJ...402..441L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Kuiper_et_al._2010,
       author = {{Kuiper}, Rolf and {Klahr}, Hubert and {Beuther}, Henrik and {Henning}, Thomas},
        title = "{Circumventing the Radiation Pressure Barrier in the Formation of Massive Stars via Disk Accretion}",
      journal = {\apj},
     keywords = {accretion, accretion disks, circumstellar matter, hydrodynamics, methods: numerical, radiative transfer, stars: formation, stars: massive, Astrophysics - Solar and Stellar Astrophysics},
         year = 2010,
        month = oct,
       volume = {722},
       number = {2},
        pages = {1556-1576},
          doi = {10.1088/0004-637X/722/2/1556},
archivePrefix = {arXiv},
       eprint = {1008.4516},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010ApJ...722.1556K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Chang_et_al.2020,
       author = {{Chang}, Philip and {Davis}, Shane W. and {Jiang}, Yan-Fei},
        title = "{Time-dependent radiation hydrodynamics on a moving mesh}",
      journal = {\mnras},
     keywords = {hydrodynamics, radiative transfer, methods: numerical, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2020,
        month = apr,
       volume = {493},
       number = {4},
        pages = {5397-5407},
          doi = {10.1093/mnras/staa573},
archivePrefix = {arXiv},
       eprint = {2002.08377},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.493.5397C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Mathis_et_al.1977,
       author = {{Mathis}, J.~S. and {Rumpl}, W. and {Nordsieck}, K.~H.},
        title = "{The size distribution of interstellar grains.}",
      journal = {\apj},
     keywords = {Cosmic Dust, Interstellar Extinction, Interstellar Matter, Particle Size Distribution, Enstatite, Graphite, Magnetite, Olivine, Polarization Characteristics, Ultraviolet Astronomy, Astrophysics},
         year = 1977,
        month = oct,
       volume = {217},
        pages = {425-433},
          doi = {10.1086/155591},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1977ApJ...217..425M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Steinacker_et_al.2010,
       author = {{Steinacker}, J. and {Pagani}, L. and {Bacmann}, A. and {Guieu}, S.},
        title = "{Direct evidence of dust growth in L183 from mid-infrared light scattering}",
      journal = {\aap},
     keywords = {dust, extinction, ISM: clouds, ISM: individual objects: L183, infrared: ISM, radiative transfer, scattering, Astrophysics - Astrophysics of Galaxies},
         year = 2010,
        month = feb,
       volume = {511},
          eid = {A9},
        pages = {A9},
          doi = {10.1051/0004-6361/200912835},
archivePrefix = {arXiv},
       eprint = {0912.0145},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010A&A...511A...9S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@book{acheson1990elementary,
  title={Elementary Fluid Dynamics},
  author={Acheson, D.J. and Acheson, F.D.J.},
  isbn={9780198596790},
  lccn={89022947},
  series={Comparative Pathobiology - Studies in the Postmodern Theory of Education},
  url={https://books.google.com/books?id=GgC69-WUTs0C},
  year={1990},
  publisher={Clarendon Press}
}


@article{Epstein1924,
  title = {On the Resistance Experienced by Spheres in their Motion through Gases},
  author = {Epstein, Paul S.},
  journal = {Phys. Rev.},
  volume = {23},
  issue = {6},
  pages = {710--733},
  numpages = {0},
  year = {1924},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRev.23.710},
  url = {https://link.aps.org/doi/10.1103/PhysRev.23.710}
}

@ARTICLE{Armitage2015,
       author = {{Armitage}, Philip J.},
        title = "{Physical processes in protoplanetary disks}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2015,
        month = sep,
          eid = {arXiv:1509.06382},
        pages = {arXiv:1509.06382},
archivePrefix = {arXiv},
       eprint = {1509.06382},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015arXiv150906382A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Birnstiel2010,
       author = {{Birnstiel}, T. and {Dullemond}, C.~P. and {Brauer}, F.},
        title = "{Gas- and dust evolution in protoplanetary disks}",
      journal = {\aap},
     keywords = {accretion, accretion disks, circumstellar matter, stars: formation, stars: pre-main sequence, infrared: stars, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2010,
        month = apr,
       volume = {513},
          eid = {A79},
        pages = {A79},
          doi = {10.1051/0004-6361/200913731},
archivePrefix = {arXiv},
       eprint = {1002.0335},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010A&A...513A..79B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Smoluchowski1916,
       author = {{Smoluchowski}, M.~V.},
        title = "{Drei Vortrage uber Diffusion, Brownsche Bewegung und Koagulation von Kolloidteilchen}",
      journal = {Zeitschrift fur Physik},
         year = 1916,
        month = jan,
       volume = {17},
        pages = {557-585},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1916ZPhy...17..557S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{JKR1971,
 ISSN = {00804630},
 URL = {http://www.jstor.org/stable/78058},
 abstract = {This paper discusses the influence of surface energy on the contact between elastic solids. Equations are derived for its effect upon the contact size and the force of adhesion between two lightly loaded spherical solid surfaces. The theory is supported by experiments carried out on the contact of rubber and gelatine spheres.},
 author = {K. L. Johnson and K. Kendall and A. D. Roberts},
 journal = {Proceedings of the Royal Society of London. Series A, Mathematical and Physical Sciences},
 number = {1558},
 pages = {301--313},
 publisher = {The Royal Society},
 title = {Surface Energy and the Contact of Elastic Solids},
 volume = {324},
 year = {1971}
}

@PHDTHESIS{S1964(JKRS),
       author = {{Sperling}, G.},
       school = {-},
         year = 1964,
        month = jan,
       adsurl = {https://ui.adsabs.harvard.edu/abs/1964PhDT.......114S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Dominik1997,
       author = {{Dominik}, C. and {Tielens}, A.~G.~G.~M.},
        title = "{The Physics of Dust Coagulation and the Structure of Dust Aggregates in Space}",
      journal = {\apj},
     keywords = {Stars: Circumstellar Matter, ISM: Dust, Extinction, Interplanetary Medium, ISM: Clouds, Solar System: Formation},
         year = 1997,
        month = may,
       volume = {480},
       number = {2},
        pages = {647-673},
          doi = {10.1086/303996},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1997ApJ...480..647D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Blum&Wurm2000,
       author = {{Blum}, J{\"u}rgen and {Wurm}, Gerhard},
        title = "{Experiments on Sticking, Restructuring, and Fragmentation of Preplanetary Dust Aggregates}",
      journal = {\icarus},
         year = 2000,
        month = jan,
       volume = {143},
       number = {1},
        pages = {138-146},
          doi = {10.1006/icar.1999.6234},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000Icar..143..138B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Paszun&Dominik2009,
       author = {{Paszun}, D. and {Dominik}, C.},
        title = "{Collisional evolution of dust aggregates. From compaction to catastrophic destruction}",
      journal = {\aap},
     keywords = {planets and satellites: formation, Astrophysics - Solar and Stellar Astrophysics},
         year = 2009,
        month = nov,
       volume = {507},
       number = {2},
        pages = {1023-1040},
          doi = {10.1051/0004-6361/200810682},
archivePrefix = {arXiv},
       eprint = {0909.3168},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009A&A...507.1023P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Voelk1980,
       author = {{Voelk}, H.~J. and {Jones}, F.~C. and {Morfill}, G.~E. and {Roeser}, S.},
        title = "{Collisions between Grains in a Turbulent Gas}",
      journal = {\aap},
     keywords = {Cosmic Dust, Interstellar Gas, Particle Collisions, Turbulence Effects, Collision Rates, Grains, Kinetic Theory, Particle Size Distribution, Protostars, Astrophysics},
         year = 1980,
        month = may,
       volume = {85},
       number = {3},
        pages = {316-325},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1980A&A....85..316V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Ormel&Cuzzi2007,
       author = {{Ormel}, C.~W. and {Cuzzi}, J.~N.},
        title = "{Closed-form expressions for particle relative velocities induced by turbulence}",
      journal = {\aap},
     keywords = {turbulence, dust, extinction, planetary systems: protoplanetary disks, Astrophysics},
         year = 2007,
        month = may,
       volume = {466},
       number = {2},
        pages = {413-420},
          doi = {10.1051/0004-6361:20066899},
archivePrefix = {arXiv},
       eprint = {astro-ph/0702303},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007A&A...466..413O},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ormel2009,
       author = {{Ormel}, C.~W. and {Paszun}, D. and {Dominik}, C. and {Tielens}, A.~G.~G.~M.},
        title = "{Dust coagulation and fragmentation in molecular clouds. I. How collisions between dust aggregates alter the dust size distribution}",
      journal = {\aap},
     keywords = {ISM: dust, extinction, ISM: clouds, turbulence, methods: numerical, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2009,
        month = aug,
       volume = {502},
       number = {3},
        pages = {845-869},
          doi = {10.1051/0004-6361/200811158},
archivePrefix = {arXiv},
       eprint = {0906.1770},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009A&A...502..845O},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{MMV1988,
       author = {{Mizuno}, H. and {Markiewicz}, W.~J. and {Voelk}, H.~J.},
        title = "{Grain growth in turbulent protoplanetary accretion disks}",
      journal = {\aap},
     keywords = {Accretion Disks, Cosmic Dust, Cosmology, Particle Size Distribution, Protoplanets, Turbulence Effects, Angular Momentum, Extrasolar Planets, Laminar Flow, Nebulae, Planetary Evolution, Solar System, Spectrum Analysis, Astrophysics},
         year = 1988,
        month = apr,
       volume = {195},
       number = {1-2},
        pages = {183-192},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1988A&A...195..183M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{TSC,
       author = {{Hockney}, R.~W. and {Eastwood}, J.~W.},
        title = "{Computer Simulation Using Particles}",
         year = 1981,
       adsurl = {https://ui.adsabs.harvard.edu/abs/1981csup.book.....H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




==> old_files/name.tex <==
\begin{equation}
  \frac{\partial E}{\partial t} + \nabla \cdot \left[ \left(E+P^*\right)\vec{v} - B\left(B \cdot \vec{v}\right) \right] = 0
\end{equation}

\begin{equation}
  \frac{\partial B}{\partial t} - \nabla \times \left[ \vec{v} \times B \right] = 0
\end{equation}

\begin{equation}
  E = \frac{P}{\gamma - 1} + \frac{\rho \left(\vec{v} \cdot \vec{v} \right)}{2} + \frac{B \cdot B}{2}
\end{equation}

\begin{equation}
  P^* = P + \frac{B \cdot B}{2}
\end{equation}



==> old_intro.tex <==

Observational evidences suggests the possibility of a substantial amount of large (mm) size grains in newly formed proto-planetary disks. The approximate flux observed as a function of frequency $\nu$ at the Rayleigh-Jeans limit is given by (Draine 2006, Beckwith 1999)
\begin{equation}
    F_\nu = \frac{2k}{c^2}\nu^2\kappa(\nu)\frac{M_dT_d}{d^2}
\end{equation}
Where k is the Boltzmann constant, c the speed of light, Md, Td are the mass and temperature of the emitting dust; d is the distance to the object. Assuming $\kappa(\nu)\propto\nu^\beta$, the observed flux $F_\nu \propto \nu^{\beta+2}$. Conventionally $\beta$ is known as the optical index and parameter $\alpha$ is defined to be $\alpha = \beta + 2$.

At mm wavelength, if the source can be resolved, the optical index at the disk can be measured. Other emission mechanisms such as free-free (e.g. Segura-Cox 2018, Karnath 2020) and synchrotron radiation (e.g. Tychoniec 2018) are either not important or can be estimated and removed using observations at other wavelengths. Tobin et. al. 2013 shows a series of observation using VLA at mm wavelength of CB230 IRS1, L1165 and L1157. The latter two objects have $\beta = 0.45\pm0.13$ and $\beta=0.6\pm0.25$ respectively. Similar results of $\beta < 1$ at mm wavelength in protoplanetary disks are shown in Kwon et al. 2015 {\color{red} more, age of these disks? L1524}. 

Natta Testi review (and citations within, Brinsteil 2018, Miyake & Nakagawa 1993) shows that if the number density of grains $n(a)$ follows a power law as a function of grain size
\begin{equation}
    n(a) \propto a^{-q}
    \label{equ:na_propto_a-q}
\end{equation}

 between $a_\mathrm{min}$ and $a_\mathrm{max}$, (Natta and Testi, 2004; etc.), then a $\beta<1$ observation suggests that $a_\mathrm{max}$ is $\geq1$mm. With $\beta < 0.5$, $a_\mathrm{max} \geq 1$cm. Assuming $a_\mathrm{min} \ll 1$mm, we can estimate the fraction of mass in grains larger than 1mm by integrating equation \ref{equ:na_propto_a-q}
 \begin{equation}
     \mathrm{fraction} = \frac{a_\mathrm{max}^{4-q} - \mathrm{1mm}^{4-q}}{a_\mathrm{max}^{4-q}}
 \end{equation}
 If we assume $q = 3.9$, with $a_max = 1$cm, $\sim30$\% of mass in grains are larger than mm. The fraction is higher with a smaller $q$.

The problem of dust coagulation in disks to produce large grains has been done over decades. People have been studing this subject from several aspects: modeling individual grain-grain interaction (JKR-S, Windmark, Wada, Blum, etc.); finding relative speeds between grains in a turbulent environment (Volk, Ormel, cuzzi & Hogan 2013, Lagrangian simulation Bate) and simulating grain dynamics in proto-planetary disks.

The essence of all grain growth simulation is the Smoluchowski equation, given by
\begin{equation}
    \frac{dn_k}{dt} = \iint_0^\infty n_in_jM_{ijk} dn_idn_j
    \label{equ:smoluchowski}
\end{equation}
where $n_i, n_j, n_k$ are the number density of grains of three sizes $s_i, s_j, s_k$; $M_{ijk}$ is the kernal decribing the result of the interaction between grain with size $s_i, s_j$. However, this equation is too complicated to be interpreted analytically due to the number inter-relation between grains of different sizes, whose properties depend their collective history of growth. Simulations have to be used to draw useful conclusions using this equation. 

Using the Smoluchowski equation in simulations, Brinsteil et. al. 2010, 2011, 2012 presents modeling of grain growth in proto-planetary disk misplane with 1-dimensional simulation, with prescribed analytical grain speeds. Similar studies on grain growth are also been done in other astrophysical settings, such as grain growth in galactic scale (e.g. Hiro, wada). 

In this work we present a 2D axis-symmetric hydrodynamical simulation of a core collapse and disk formation, and post-process the hydrodynamical simulation to study dust dynamics and grain growth in newly formed protoplanetary disks. The setups of the hydrohydamical simulation and dust simulation are shown in section \S~\ref{sec:setup}. An overlook of the hydrodynamic disk is shown in section \S~\ref{sec:hydro_results}. In section \S~\ref{sec:dust_the_fiducial_model} we show that drift velocities alone cannot lead to substantial grain growth to produce the grains seen in observation. An increase in growth rate is necessary to produce the large grains and we will discuss some properties of the dust disk we obtain in the simulation in section \S~\ref{sec:dust_the_chi=4_model}. Ways to get the increased growth rate is discussed in section \S~\ref{sec:increase_grain_growth_rate}. We conclude in section \S~\ref{sec:conclusion}.


Motivation
\begin{enumerate}
    \item Origin of planets still unknown
    \item grain growth as seeds for planets
    \item observational evidence for large grains in early Class 0 disks from VLA observations (e.g., L1527, NGC 1333 IRAS4a, Orion sources (Nicole Karnash et al), and VANDAM VLA survey in general). Amount of large grains needed to explain the observed VLA flux? How to grow these grains within the available time and given the dynamical constraints (envelope to disk transition)?
    \item{100 micron grains from scattering}
    \item The Smoluchowski equation used to model grain growth is very hard to draw useful conclusion without simulation because of the number of variables.
\end{enumerate}

==> old_turbulence.tex <==
\section{Possible ways to get an increased grain growth rate}
\label{sec:increase_grain_growth_rate}
{\color{red} Plot the ratio in the last panel for all 20 cells in the one-cell simulation, and argue what structure would we see if no drift.}
One potential way to get an increase in grain growth rate is to increase grain-grain relative speed via sub-grid turbulence. \citet{Voelk1980} presented the relative speeds between grains of different sizes in a turbulent environment. The environment is described by assuming a largest turbulence scale $L_g$ and a series of eddies whose energies are described by the Kolmogorov cascade. \citet{MMV1988} and \citet{OrmelCuzzi2007} improved the theory and \citet{Ormel2009} came forward with a grain growth model using this relative speed theory.

In \citet{Birnstiel2010}, one-dimensional proto-planetary disk grain coagulation simulations are conducted using a prescribed speed to represent the bulk motion, and includes the relative speeds induced by the turbulence model. In figure \ref{fig:speed_compare_with_Brinsteil} we present a comparison between grain-grain relative speed in a cell calculated in our simulation and analytical relative speed using equations found in \citet{Birnstiel2010}. The cell we present here is chosen to be {\color{red} the fiducial cell used in the one-cell models (located at 26AU on the midplane)}, while other midplane cells leads to the same conclusion. The bulk relative speeds, as shown in the first and second column, have similar behavior in both simulations. Brownian motion, as discussed in section \ref{sec:Grain_spatial_transportation}, has negligible contributions except for grains with the smallest sizes. Sub-grid turbulence, however, can cause a significant increase in grain relative speeds. The right lower panel shows the sum of analytic relative speeds and turbulence induced relative speeds divided by relative speeds in our simulation. The difference is as high as $1000$ times for small grain-small grain interaction and a factor of $3\sim 5$ for interactions involving large, $>$mm size grains.

In figure \ref{fig:vertical_density_compare_Brinsteil} we show the vertically integrated surface density of grains of different sizes in the disk of the $\chi=4$ model. We compare our results with figure 5 in \citet{Birnstiel2010}. Note that only part of figure 5 in \citet{Birnstiel2010} is comparable to our result, from 10AU to 200 AU and dust size from $10^{-5}\to 10^0$ cm. We see a similar size-layering in both our model and Brinsteil's model, but \citet{Birnstiel2010} gets more large grains than we do. The result is expected given the increased grain growth rate due to including turbulence-induced relative speeds.
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{figures/74_40_speed_compare_with_brinsteil_r45theta103.png}
    \caption{An example of pairwise grain-grain relative speeds in each direction in the spherical-polar coordinate. The first and second column are the relative speeds in each direction and total relative speeds found in our simulation and analytically derived value as used in \citet{Birnstiel2010} respectively. On the third column we plot the inferred relative speeds due to turbulence (see \citet{Voelk1980}, \citet{OrmelCuzzi2007}). The colored plot on the right lower corner shows the ratio between the values would have been used in \citet{Birnstiel2010} if the cell were in his simulation, and the calculated value in our simulation. As we can see the turbulence induced relative speed is much larger than the drift-induced relative speeds for cells on the midplane.}
    \label{fig:speed_compare_with_Brinsteil}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{figures/74_40_Brinsteil.png}
    \caption{Caption}
    \label{fig:vertical_density_compare_Brinsteil}
\end{figure*}
